Bridging the Gap between Constant Step Size Stochastic Gradient Descent and Markov Chains

We consider the minimization of an objective function given access to unbiased estimates of its gradient through stochastic gradient descent (SGD) with constant step-size. While the detailed analysis was only performed for quadratic functions, we provide an explicit asymptotic expansion of the moments of the averaged SGD iterates that outlines the dependence on initial conditions, the effect of noise and the step-size, as well as the lack of convergence in the general (non-quadratic) case. For this analysis, we bring tools from Markov chain theory into the analysis of stochastic gradient. We then show that Richardson-Romberg extrapolation may be used to get closer to the global optimum and we show empirical improvements of the new extrapolation scheme.

==> header.tex <==



\newcommand{\tcr}[1]{\textcolor{red}{#1}}
\newcommand{\tcb}[1]{\textcolor{blue}{#1}}

%\PassOptionsToPackage{numbers, compress}{natbib}



%\usepackage{nips_2017}
% \setlength{\bibsep}{0pt plus 0.3ex}

% to compile a camera-ready version, add the [final] option, e.g.:
% \usepackage[final]{nips_2016}

\usepackage[utf8]{inputenc}
%\usepackage[T1]{fontenc}    % use 8-bit T1 fonts
\usepackage{url}            % simple URL typesetting
\usepackage{booktabs}       % professional-quality tables
%\usepackage{nicefrac}       % compact symbols for 1/2, etc.
\usepackage{microtype}      % microtypography

%\documentclass[nolayout,preprint]{imsart}
%\documentclass[nolayout,a4,10pt]{imsart}
%\RequirePackage[OT1]{fontenc}
\RequirePackage{amsmath}
%\RequirePackage[numbers]{natbib}
%\RequirePackage[colorlinks,citecolor=blue,urlcolor=blue]{hyperref}

%\usepackage[a4paper]{geometry} % required for statsoc+pdflatex


% \usepackage[notref,notcite]{showkeys}  %  comment out for final version
% \renewcommand*\showkeyslabelformat[1]{\fbox{\normalfont\scriptsize\sffamily#1}}   % for showkeys


\usepackage{stmaryrd}


\usepackage{amsthm}
\usepackage{amssymb}
\usepackage{makeidx}
\usepackage[english]{babel}
\usepackage{graphicx}
\usepackage{amsfonts,amssymb}
%\usepackage{epstopdf}
%\usepackage{lmodern}
\usepackage{oldgerm}
%\usepackage{euler}
\usepackage{mathrsfs}
\usepackage[active]{srcltx}
\usepackage{verbatim}
\usepackage{enumitem, kantlipsum} %label option for enumerate \alph* \Alph* \roman* \Roman* or other... [label=$\bullet$], [label=\alph*]usepackage{enumitem,}
%\usepackage[comma,authoryear,longnamesfirst]{natbib}
%\usepackage[authoryear]{natbib}
%\usepackage{enumerate}
%\usepackage[toc,page]{appendix}
\usepackage{aliascnt}
\usepackage{bbm}
\usepackage{array}
\usepackage{hyperref}
\hypersetup{colorlinks=true,citecolor=blue, urlcolor=blue, linkcolor=red, filecolor=black}
%\usepackage[ruled,vlined]{algorithm2e}
%\usepackage[textwidth=4cm,textsize=footnotesize]{todonotes}
 \usepackage[disable]{todonotes}
\usepackage{xargs}
\usepackage{cellspace}
\usepackage{xr}

\usepackage[Symbolsmallscale]{upgreek}
%\usepackage{environ}

\usepackage[algo2e,inoutnumbered,algoruled,vlined]{algorithm2e} %linesnumbered
\usepackage{xcolor}
\definecolor{mydarkblue}{rgb}{0,0.08,0.45}
\usepackage{multicol} 
% \setlength{\multicolsep}{6.0pt plus 2.0pt minus 1.5pt}
\setlength{\multicolsep}{0.1pt plus 1pt minus 1.5pt}


\usepackage{subcaption} 
\usepackage{wrapfig}

%\usepackage[novbox]{pdfsync}           %  [novbox] helps

% \usepackage{vwcol}

%\usepackage{vmargin} % required for statsoc+pdflatex

\usepackage{accents}
\usepackage{dsfont}
\usepackage{aliascnt}
\usepackage{cleveref}
\makeatletter
\newtheorem{theorem}{Theorem}
\crefname{theorem}{theorem}{Theorems}
\Crefname{Theorem}{Theorem}{Theorems}


\newtheorem*{lemma_nonumber*}{Lemma}


\newaliascnt{lemma}{theorem}
\newtheorem{lemma}[lemma]{Lemma}
\aliascntresetthe{lemma}
\crefname{lemma}{lemma}{lemmas}
\Crefname{Lemma}{Lemma}{Lemmas}



\newaliascnt{corollary}{theorem}
\newtheorem{corollary}[corollary]{Corollary}
\aliascntresetthe{corollary}
\crefname{corollary}{corollary}{corollaries}
\Crefname{Corollary}{Corollary}{Corollaries}

\newaliascnt{proposition}{theorem}
\newtheorem{proposition}[proposition]{Proposition}
\aliascntresetthe{proposition}
\crefname{proposition}{proposition}{propositions}
\Crefname{Proposition}{Proposition}{Propositions}

\newaliascnt{definition}{theorem}
\newtheorem{definition}[definition]{Definition}
\aliascntresetthe{definition}
\crefname{definition}{definition}{definitions}
\Crefname{Definition}{Definition}{Definitions}

\newaliascnt{remark}{theorem}
\newtheorem{remark}[remark]{Remark}
\aliascntresetthe{remark}
\crefname{remark}{remark}{remarks}
\Crefname{Remark}{Remark}{Remarks}


\newtheorem{example}[theorem]{Example}
\crefname{example}{example}{examples}
\Crefname{Example}{Example}{Examples}


\crefname{figure}{figure}{figures}
\Crefname{Figure}{Figure}{Figures}


%\newtheorem{assumption}{\textbf{A}\hspace{-3pt}}
%\Crefname{assumption}{\textbf{A}\hspace{-3pt}}{\textbf{A}\hspace{-3pt}}
%\crefname{assumption}{\textbf{A}}{\textbf{A}}
\newtheorem{assumption}{\textbf{A}\hspace{-3pt}}
\crefformat{assumption}{{\textbf{A}}#2#1#3}





\newtheorem{assumptionG}{\textbf{G}\hspace{-3pt}}
\Crefname{assumptionG}{\textbf{G}\hspace{-3pt}}{\textbf{G}\hspace{-3pt}}
\crefname{assumptionG}{\textbf{G}}{\textbf{G}}

\newtheorem{assumptionQ}{\textbf{Q}\hspace{-3pt}}
\Crefname{assumptionQ}{\textbf{Q}\hspace{-3pt}}{\textbf{Q}\hspace{-3pt}}
\crefname{assumptionQ}{\textbf{Q}}{\textbf{Q}}

\newcounter{cmtcounter}
\setcounter{cmtcounter}{1}
\newcommand{\cmt}[1]{\textcolor{magenta}{[\arabic{cmtcounter}]
    \textit{#1}}\addtocounter{cmtcounter}{1}}
\newcommand{\cmtbox}[1]{
  \begin{center}
    \fbox{
      \begin{minipage}{.8\columnwidth}
        \textcolor{magenta}{[\arabic{cmtcounter}] \textit{#1}}
      \end{minipage}
    }
  \end{center}
  \addtocounter{cmtcounter}{1}}


% ADD THE FOLLOWING COUPLE LINES INTO YOUR PREAMBLE
\let\OLDthebibliography\thebibliography
\renewcommand\thebibliography[1]{
  \OLDthebibliography{#1}
  \setlength{\parskip}{2.0pt}
  \setlength{\itemsep}{1pt plus 1ex}
}


%%%%%Comment figures
% \usepackage{comment}
% \excludecomment{figure}
% \let\endfigure\relax

% \excludecomment{wrapfigure}
% \let\endwrapfigure\relax

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../main"
%%% End:

